milliMamba: Specular-Aware Human Pose Estimation via Dual mmWave Radar with Multi-Frame Mamba Fusion

Millimeter-wave radar offers a privacy-preserving and lighting-invariant alternative to RGB sensors for Human Pose Estimation (HPE) task. However, the radar signals are often sparse due to specular reflection, making the extraction of robust features from radar signals highly challenging. To address this, we present milliMamba, a radar-based 2D human pose estimation framework that jointly models spatio-temporal dependencies across both the feature extraction and decoding stages. Specifically, given the high dimensionality of radar inputs, we adopt a Cross-View Fusion Mamba encoder to efficiently extract spatio-temporal features from longer sequences with linear complexity. A Spatio-Temporal-Cross Attention decoder then predicts joint coordinates across multiple frames. Together, this spatio-temporal modeling pipeline enables the model to leverage contextual cues from neighboring frames and joints to infer missing joints caused by specular reflections. To reinforce motion smoothness, we incorporate a velocity loss alongside the standard keypoint loss during training. Experiments on the TransHuPR and HuPR datasets demonstrate that our method achieves significant performance improvements, exceeding the baselines by 11.0 AP and 14.6 AP, respectively, while maintaining reasonable complexity. Code: https://github.com/NYCU-MAPL/milliMamba

==> table/ablation_different_model.tex <==
% ablation table -- different model
\begin{table}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c c c c c c c c|c c c|}
\hline
\textbf{Network} & \multicolumn{8}{c|}{\textbf{Joint-wise AP}} & \multicolumn{3}{c|}{\textbf{Overall AP}} \\
 & Head & Neck & Shoulder & Elbow & Wrist & Hip & Knee & Ankle & AP & AP$^{50}$ & AP$^{75}$ \\
\hline\hline
mmPose~\cite{mmpose} & 54.4 & 61.5 & 50.8 & 35.4 & 17.4 & 82.9 & 72.7 & 62.7 & 51.7 & 91.5 & 50.2 \\
HuPR~\cite{hupr} &  &  &  &  &  &  &  &  &  &  &  \\
TransHuPR~\cite{transhupr} & 79.2 & 82.8 & 75.9 & 56.9 & 40.3 & 91.5 & 84.8 & 78.1 & 73.7 & 97.3 & 84.3 \\
Ours & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
\hline
\end{tabular}
}
\end{center}
\caption{}
\label{tab:ablation_different_model_AP}
\end{table}

==> table/ablation_mamba_scan.tex <==
%% ablation table -- input modality
\begin{table}
\caption{Ablation study on the impact of different mamba scanning patterns.}
\label{tab:ablation_mamba_scanning_AP}
\centering
\begin{tabular}{c|ccc}
\hline
\textbf{Scanning Pattern in Mamba} & AP & AP$^{50}$ & AP$^{75}$ \\ \hline
Spiral Scan & 70.8 & 97.0 & 80.8 \\
\textit{frame} \(\rightarrow\) \textit{range} \(\rightarrow\) \textit{angle} & 72.1 & 97.2 & 81.4 \\
\textit{angle} \(\rightarrow\) \textit{range} \(\rightarrow\) \textit{frame} & 72.6 & 97.3 & 82.7 \\
\textit{range} \(\rightarrow\) \textit{angle} \(\rightarrow\) \textit{frame} & \textbf{74.5} & \textbf{98.5} & \textbf{84.7} \\ \hline
\end{tabular}
\end{table}
